Benchmarking Potential Based Rewards for Learning Humanoid Locomotion

The main challenge in developing effective reinforcement learning (RL) pipelines is often the design and tuning the reward functions. Well-designed shaping reward can lead to significantly faster learning. Naively formulated rewards, however, can conflict with the desired behavior and result in overfitting or even erratic performance if not properly tuned. In theory, the broad class of potential based reward shaping (PBRS) can help guide the learning process without affecting the optimal policy. Although several studies have explored the use of potential based reward shaping to accelerate learning convergence, most have been limited to grid-worlds and low-dimensional systems, and RL in robotics has predominantly relied on standard forms of reward shaping. In this paper, we benchmark standard forms of shaping with PBRS for a humanoid robot. We find that in this high-dimensional system, PBRS has only marginal benefits in convergence speed. However, the PBRS reward terms are significantly more robust to scaling than typical reward shaping approaches, and thus easier to tune.

==> Sections/equivalences.tex <==
\section{Regularization and Equivalences}
We take the view that a proxy reward function acts as a regularizer to guide the policy gradients toward the optimal policy.
A perfect regularizer provides strong reward signal everywhere, and always points towards the true optimal policy.
In such a case, the regularizer does not affect the optimal solution.

We take the specific case of greedy policies (discount factor $\gamma = 0$) to compare regularization capability.
The intuition, similar to GAE SCHULMAN, is to treat the $\gamma$ as a tunable parameter that "weights" the proxy reward against the sparse reward. This becomes true especially if $R_{sparse} >> R_{proxy}$.
Clearly, the true value function is a perfect regularizer: regardless of the state, the greedy action is an optimal policy.
Thus, substituting the reward with the true optimal value function is adding a perfect regularizer, yay.
The PBRS is not necessary, but has a favorable property: it keeps the value reasonable everywhere, since it "cancels out" increments.
This has advantages: it doesn't lose the invariance property for other potential functions (including approximations of the value function).
\par
We note that common reward terms such as reference tracking or energy-pumping are a subclass of potential functions.
In these cases, we have $\Phi(s) = ||p(s) - p_(s_{\text{des}})||$, where $|| ||$ is a norm, $p$ is a function (not functional).
For example, standard reference tracking in joint-space, $p$ is the identity, and $s_{\text{des}}(t)$ is a reference tracking.
For energy pumping, $p$ is the total energy, and $s_{\text{des}}$ is a constant representing the total energy at inverted rest.
\par
As potential functions, they can naturally be used in the PBRS setting.
We note that with $\gamma = 0$, we have
\begin{align}
    \tilde{r} & = \Phi(s') - \Phi(s)
    & = ||p(s') - p_(s'_\text{des})|| - ||p(s) - p_(s_\text{des})||
\end{align}
which is essentially rewarding the finite-difference of the error.
In other words, instead of directly rewarding a small error, it rewards the rate at which the error decreases.
In other (other) words, the reward is working at the level of the error dynamics.
\par
We conjecture that in many practical cases, it is easier to specify a potential function that is similar at the level of the error-dynamics, despite large mismatches in distance.

% Show that PBRS and direct reward shaping (DRS) using the true optimal value do not affect results (in theory).
% Corner case: greedy PBRS (discount factor $\gamma=0$) is the same as tracking the potential function.

% Case: reference trajectory as DRS and PBRS. With PBRS, moving to the error dynamics, and essentially looking at the first order finite differences. Provides a slightly better metric.
% SIDE THOUGHT do other integration schemes still maintain NG's invariance properties in theory? I suppose if you looked at this as the discretization of the continuous-time version, it probably would pop out.



==> Sections/pendulum.tex <==


\section{Inverted Pendulum Case Study}
We begin by evaluating the effects of using potential-based rewards on a simple pendulum system for a swing-up task.
The inverted pendulum is a particularly attractive case study because we can directly visualize the rewards seen by the agent, the value function, and the policy in two dimensions.

\subsection{Experiments}
For a simple pendulum system with mass $m$, gravity $g$, length $l$, and state $s$, we consider several different training scenarios to highlight the effects of using potential-based rewards.
We define our "actual" reward for the task as follows:
\begin{align}
    r_{true}(s_k) &= 
    \begin{cases}
        10, & \lvert \theta_k \rvert \leq 0.05 \: \operatorname{and} \: \lvert \dot{\theta_k} \rvert \leq 0.1 \\
        0, & \operatorname{otherwise}.
    \end{cases}
\end{align}
For this low-dimensional system, an optimal policy can be found even with this sparse reward, but we wish to compare the effects of regularization between typical reward shaping and PBRS. 
To that end, we consider the following cases:
\sehwan{Can add to/edit these cases as needed}
\begin{subequations}
    \label{eq:pend_cases}
    \begin{align}
        r_{shaping}(s_k) &= (E(s_k) - E_d)^2, \\
        \hat{r}_{shaping}(s_k) &= (E(s_k) - 2E_d)^2, \\
        r_{PB}(s_k, s_{k+1}) &= \gamma r_{shaping}(s_{k+1}) - r_{shaping}(s_k), \\
        \hat{r}_{PB}(s_k, s_{k+1}) &= \gamma \hat{r}_{shaping}(s_{k+1}) - \hat{r}_{shaping}(s_k),
    \end{align}
\end{subequations}

where $r_{shaping}$ and $r_{PB}$ are the shaping and potential-based rewards respectively, and $E(s)$ and $E_d = mgl$ are the energy of the state and desired energy at vertical respectively.
\par

We choose to use "energy-pumping" rewards as a dense reward signal for the swing-up task, as in~\cite{Astrom_PendEnergyPumping}.
To compare the effects of using rewards and potential-based rewards to "erroneous" regularization, $\hat{r}_{shaping}$ and $\hat{r}_{PB}$ penalizes the deviation from \emph{double} the energy of the pendulum in the upright position.

\subsection{Implementation}
\sehwan{Steve, you might want to detail this part, not 100\% sure how Vibly works.} \\
Each of the rewards in Eq.~\ref{eq:pend_cases} are added to $r_{true}$ and solved with Q-Value iteration with the \texttt{Vibly} package. 
State space + action space discretization, training gamma, PBRS gamma, other details.
The training is ran until a tolerance threshold of [] is met.


\subsection{Results}

For the pendulum system, we show the rewards, converged value function, and converged policy for each set of the rewards outlined in Eq.~\ref{eq:pend_cases} in Fig.~\ref{fig:pend_caseStudy}.
With tabular Q-Value iteration, the theoretical guarantees from \cite{Ng_PolicyInvariance} are consistent with the results found.
With the potential-based rewards, the optimal policy found is nearly identical to that of the policy with only the "true" rewards, \emph{regardless} of the quality of regularization.
Comparing Fig.~\ref{fig:pend_caseStudy}c. and e., even when rewarding an incorrect desired energy, using the potential-based form of the rewards causes convergence to the original optimal policy.
\par

In contrast, using typical reward shaping for the pendulum system causes significant deviation from the optimal policy.
As expected, the optimal policy is affected, but well regularized near the optimal policy in Fig.~\ref{fig:pend_caseStudy}b. and poorly regularized in Fig.~\ref{fig:pend_caseStudy}d. 
\par

\sehwan{There's more to say about this, and better, but I'm going to move on to writing about the humanoid so we can see how much space we have.}

In summary, we demonstrate that potential-based rewards seem more \emph{robust} to incorrect regularization, and does not affect the optimal policy, at least for this low-dimensional case study.
While the incorrect rewards in Eq.~\ref{eq:pend_cases} are somewhat contrived, the key insight is that if the learning process is \emph{robust} to the designed rewards, finding a desirable policy becomes much easier.
\par

For high-dimensional systems, it is much less clear how to design rewards to regularize the agent's behavior without significantly modifying it.
Consequently, formulating the reward function involves laborious tuning, designing, and balancing to manage this tradeoff.

\sehwan{maybe a paper that has a complicated rwd function as an example}.

\sehwan{This last part is messy, need to reword.}

% PROBABLY KICK (at least) ONE OF THESE.
% \par
% Show case parsimonious reward value function, used as DTRS with $\gamma = 0$, and PBRS.
% The perturb value function and evaluate effect.
% \par
% Use approximate cost-to-go in the form of Q cost, and show the dependency on choice of Q, in DTRS vs PBRS.
% \par
% Use energy-shaping as DTRS and PBRS, and show robustness with respect to choice of desired energy.
% \par
% Use an optimal trajectory as DTRS and PBRS. Compare resulting optimal paths compared to true optimal.
% \par
% Show how the regularizing property changes in function to \emph{qualitative} changes in vector field (and thus error dynamics).
% Does PBRS enjoy benefits?
